Improving Neural Network Quantization without Retraining using Outlier Channel Splitting

Quantization can improve the execution latency and energy efficiency of neural networks on both commodity GPUs and specialized accelerators. The majority of existing literature focuses on training quantized DNNs, while this work examines the less-studied topic of quantizing a floating-point model without (re)training. DNN weights and activations follow a bell-shaped distribution post-training, while practical hardware uses a linear quantization grid. This leads to challenges in dealing with outliers in the distribution. Prior work has addressed this by clipping the outliers or using specialized hardware. In this work, we propose outlier channel splitting (OCS), which duplicates channels containing outliers, then halves the channel values. The network remains functionally identical, but affected outliers are moved toward the center of the distribution. OCS requires no additional training and works on commodity hardware. Experimental evaluation on ImageNet classification and language modeling shows that OCS can outperform state-of-the-art clipping techniques with only minor overhead.

==> fig-runtime.tex <==
\begin{figure}[thb]
  \begin{center}
  \includegraphics[width=\columnwidth, trim=40 40 40 40]{fig-runtime-plot.pdf}
  \vskip -0.2in
  \caption{\BF{CNN wallclock inference time with OCS --} the x-axis shows different expand ratios, with zero being the baseline and non-zeros utilizing additional code for weight OCS. Runtime is measured for inference over the entire test set with batch size 128 on an NVIDIA GTX 1080 Ti.
  }
  \label{fig:runtime}
  \end{center}
  \vspace{-10px}
\end{figure}

==> tab-ocs-acts-cifar10-resnet.tex <==
\begin{table}[tb]
    \centering
    \caption{CIFAR-10 accuracy on ResNet-20 when quantizing both weights and activations with different expansion ratios. Both weights and activations use 4 bits.}
    \begin{tabular}{c|cccc}
    \toprule
        \multirow{2}[0]{*}{\BF{OCS on Weights}} & \multicolumn{4}{c}{\BF{OCS on Activations}} \\
        & \BF{0.0} & \BF{0.01} & \BF{0.02} & \BF{0.05} \\
    \midrule
    \BF{0.0} & 63.56 & 67.70 & 67.72 & 67.41 \\
    \midrule
    \BF{0.01} & 64.82 & 68.85 & 68.98 & 68.86 \\
    \midrule
    \BF{0.02} & 64.98 & 69.36 & 68.85 & 69.61 \\
    \midrule
    \BF{0.05} & 66.85 & 70.23 & 70.23 & 70.22\\
    \bottomrule
    \end{tabular}
    \label{tab:ocs-acts-cifar10-resnet}
\end{table}

